Flow Matching with Optimized Subclass Priors for Medical Image Augmentation

Rare diseases dominate the diagnostic challenge in medical imaging yet are severely underrepresented in clinical datasets, causing classifiers to fail on exactly the conditions where reliable detection matters most. Generative augmentation can supply the missing tail-class coverage, but coarse disease labels aggregate diverse subtypes and acquisition settings into multi-modal conditionals that bias generators toward dominant submodes, while a shared Gaussian source forces rare subpopulations through disproportionately long transport paths. We propose an offline strategy that introduces informative priors at two levels: first, we partition each coarse label into coherent submodes via Gaussian mixture modeling in the generative model's latent space; second, we learn subclass-conditioned source distributions that re-center and re-scale the starting distribution per submode, shortening trajectories and reducing within-subclass dispersion. To prevent degenerate solutions we impose explicit geometric control, moderately concentrating normalized displacement directions around learnable prototypes while capping path-length outliers. On long-tailed chest X-ray (MIMIC-LT, NIH-LT) and CT slice (CT-RATE) benchmarks the proposed method consistently improves tail-class generation fidelity and diversity (FID, IRS) and is a promising augmentation strategy that reliably improves downstream balanced accuracy and macro-F1 over a non-augmented baseline across modalities.

==> figures/balanced_geo.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/balance.pdf}
    \caption{\textbf{Left:} Overly close sourcs produce noisy directions, while sources which are too far produce entangled paths. \textbf{Right:} Our method balances angular concentration and distance to targets.}
    \label{fig:bal_geo}
\end{figure}

==> figures/synth.tex <==
\begin{figure*}[t]
\centering
\newcommand{\w}{0.19\textwidth}

\includegraphics[width=\w]{images/source_A.pdf}\hfill
\includegraphics[width=\w]{images/gen_A.pdf}\hfill
\includegraphics[width=\w]{images/target.pdf}\hfill
\includegraphics[width=\w]{images/source_B.pdf}\hfill
\includegraphics[width=\w]{images/gen_B.pdf}

\vspace{1mm}
{\scriptsize (a) $\mathcal{N}(0,I)$ Source}\hfill
{\scriptsize (b) Generated 1}\hfill
{\scriptsize (c) Target}\hfill
{\scriptsize (d) Subclass Priors}\hfill
{\scriptsize (e) Generated 2}

\caption{Left-to-right comparison of using a single zero mean Gaussian against our method with the same seed on unbalanced synthetic 2D checkerboard data.}
\label{fig:synth}
\end{figure*}


==> tables/ablation.tex <==
\begin{table}[htbp]
\centering
\caption{Classifier ablation on augmented training data (bAcc mean$\pm$std across nine seeds).}
\label{tab:cls_ablation_mimic_ctrate}
\begin{tabular}{cccc}
\toprule
Subclasses & Optimization & MIMIC-LT & CT-RATE \\
\midrule
 &  & $0.149_{\pm0.008}$ & $\underline{0.191_{\pm0.012}}$ \\
 & \checkmark & $\underline{0.158_{\pm0.007}}$ & $0.173_{\pm0.016}$ \\
\checkmark &  & $\underline{0.158_{\pm0.006}}$ & $0.182_{\pm0.017}$ \\
\checkmark & \checkmark & $\mathbf{0.162_{\pm0.005}}$ & $\mathbf{0.193_{\pm0.014}}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/classifier.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{5.5pt}
\caption{Classifier results for MIMIC-LT and CT-RATE (mean$\pm$std). Real denotes real-only classifier training, the other methods are a mix of real and synthetic images. Best results per column are in bold, while second best are underlined.}
\label{tab:cls_results}
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{MIMIC-LT} & \multicolumn{2}{c}{CT-RATE} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Method & bAcc $\uparrow$ & Macro-F1 $\uparrow$ & bAcc $\uparrow$ & Macro-F1 $\uparrow$ \\
\midrule
Real & $0.157\!_{\pm0.014}$ & $0.158\!_{\pm0.013}$ & $0.176\!_{\pm0.009}$ & $0.164\!_{\pm0.012}$ \\
Vanilla & $0.149\!_{\pm0.008}$ & $0.153\!_{\pm0.008}$ & $\underline{0.191\!_{\pm0.012}}$ & $0.171\!_{\pm0.023}$ \\
CBFM~\cite{qin2023cb} & $0.150\!_{\pm0.009}$ & $0.153\!_{\pm0.009}$ & $0.179\!_{\pm0.017}$ & $0.165\!_{\pm0.019}$ \\
CPD~\cite{issachar2025designing} & $\underline{0.159\!_{\pm0.013}}$ & $\underline{0.159\!_{\pm0.017}}$ & $0.189\!_{\pm0.012}$ & $\underline{0.173\!_{\pm0.014}}$ \\
Ours & $\mathbf{0.162\!_{\pm0.005}}$ & $\mathbf{0.163\!_{\pm0.006}}$ & $\mathbf{0.193\!_{\pm0.014}}$ & $\mathbf{0.177\!_{\pm0.011}}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/metrics.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{5.0pt}
\caption{Macro generative metrics using dataset-specific local feature extractors: local CXR for MIMIC-LT and local CT-RATE DenseNet for CT-RATE. Values are mean$\pm$std across seeds. Best per metric is bold; second best is underlined.}
\label{tab:macro_metrics_mimic_ctrate}
\begin{tabular}{lcccc}
\toprule
Method & \multicolumn{2}{c}{MIMIC-LT} & \multicolumn{2}{c}{CT-RATE} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& FID$_{\text{train}}\downarrow$ & IRS$\uparrow$ & FID$_{\text{train}}\downarrow$ & IRS$\uparrow$ \\
\midrule
Vanilla & $0.0478\!_{\pm0.0021}$ & $0.6150\!_{\pm0.0173}$ & $\underline{27.106\!_{\pm1.248}}$ & $0.6935\!_{\pm0.0223}$ \\
CBFM & $\underline{0.0468\!_{\pm0.0027}}$ & $\underline{0.6255\!_{\pm0.0199}}$ & $\mathbf{27.004\!_{\pm0.938}}$ & $\mathbf{0.7129\!_{\pm0.0191}}$ \\
CPD & $0.0516\!_{\pm0.0029}$ & $0.5644\!_{\pm0.0066}$ & $28.475\!_{\pm0.695}$ & $0.6712\!_{\pm0.0392}$ \\
Ours & $\mathbf{0.0446\!_{\pm0.0004}}$ & $\mathbf{0.6676\!_{\pm0.0105}}$ & $29.056\!_{\pm0.356}$ & $\underline{0.7124\!_{\pm0.0222}}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/optimization_diagnostics.tex <==
\begin{table}[htbp]
  \centering
  \label{tab:geom_diag}
  \caption{Geometric diagnostics (before $\rightarrow$ after source optimization):
  directional alignment $\cos_{\mathrm{mean},w}$ and normalized radial variability $r_{\mathrm{rel},w}$ are shown.} 
  \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{lcc}
      \toprule
      Dataset & $\cos_{\mathrm{mean},w}$ & $r_{\mathrm{rel},w}$\\
      \midrule
      MIMIC-LT    & $0.00 \rightarrow 0.68\;(+0.68)$ & $0.08 \rightarrow 0.04\;(-46\%)$ \\
      CT-RATE     & $0.00 \rightarrow 0.69\;(+0.69)$ & $0.07 \rightarrow 0.03\;(-57\%)$ \\
      \bottomrule
    \end{tabular}%
  }
\end{table}


==> tables/subclass.tex <==
\begin{table}[htbp]
  \centering
  \caption{Split summary for priors based on the EBIC criterion.
  $B$ = #base classes, $K$ = #subclasses.
  ``\sout{split}'' means base class with $K_c=1$; ``split'' means $K_c>1$.}
  \label{tab:subclass}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{lcccccc}
  \toprule
  Dataset & $B$ & $K$ & \#\sout{split} & |\sout{split}\textsubscript{max}|  & |split\textsubscript{min}| & $\min n_{c,k} \in $ split \\
  \midrule
  MIMIC-LT    & 19 & 91 & 6 & 254 & 609 & 106 \\
  CT-RATE     & 15 & 53 & 7 & 244 & 335 & 97 \\
  \bottomrule
  \end{tabular}%
  }
\end{table}


==> tables/subclass_structure.tex <==
\begin{table}[htbp]
  \centering
  \small
  \caption{Weighted (by class sample count) kNN purity for learned subclasses versus matched random partitions.}
  \begin{tabular}{lcccc}
  \toprule
  Embedding space & kNN purity (subclass) $\uparrow$ & kNN purity (random baseline) & $\Delta$kNN $
  \uparrow$ \\
  \midrule
  CXR Densenet~\cite{dombrowski2026pso} & 0.295 & 0.131 & 0.164 \\
  BioViL~\cite{boecking2022biovil}    & 0.231 & 0.131 & 0.100 \\
  \bottomrule
  \end{tabular}
  \label{tab:kknn_subclass_vs_random}
  \end{table}

